Synergistic Integration of Optical and Microwave Satellite Data for Crop Yield Estimation

Developing accurate models of crop stress, phenology and productivity is of paramount importance, given the increasing need of food. Earth observation remote sensing data provides a unique source of information to monitor crops in a temporally resolved and spatially explicit way. In this study, we propose the combination of multisensor (optical and microwave) remote sensing data for crop yield estimation and forecasting using two novel approaches. We first propose the lag between Enhanced Vegetation Index derived from MODIS and Vegetation Optical Depth derived from SMAP as a new joint metric combining the information from the two satellite sensors in a unique feature or descriptor. Our second approach avoids summarizing statistics and uses machine learning to combine full time series of EVI and VOD. This study considers two statistical methods, a regularized linear regression and its nonlinear extension called kernel ridge regression to directly estimate the county-level surveyed total production, as well as individual yields of the major crops grown in the region: corn, soybean and wheat. The study area includes the US Corn Belt, and we use agricultural survey data from the National Agricultural Statistics Service (USDA-NASS) for year 2015 for quantitative assessment.

==> weight_models.tex <==
\red{tenim analisis de feonologia amb metode LASSO i RLR pero no acabem de interpretar-ho. Ara tambe tenim els pesos (alpha) de cada county segons KRR (Figura \ref{fig:weigthKRR}). He afegit informacio de crop prop i lva produccio dels counties en major i menor valor de alpha per veure si podem treure alguna conclusio. }


The phenological metrics provide knowledge about the ecosystem and the growing progress of the crops. The vegetation indices we used are capable to represent this progress and also discriminate what type of cropland we find in each county, but the peculiarity of our experiments is that we can use a fixed time series without having to define the different phases of the phenological vegetation along the year. In this section we analyze if the methods are able to place value on. 

The importance of the input variables (i.e., the predictors) were ranked with the LASSO method for EVI \& VOD in each experiment. Due to the combination of both vegetation indices obtained the best results, we studied how the model interprets EVI and VOD data according to the output crop.

LASSO method performs the variable selection (i.e. does not use all input matrix), and establishes coefficients or weights like the linear regression method. The advantage of LASSO is the non-utilization of all variables,  facilitating analysis and understanding of the importance of the input variables. The values of the weights of the LASSO methods can be interpreted as a proxy to the importance of each input variable, where variables associated with larger weights have more importance in the final prediction. In Tab. \ref{tab:resultsLASSO} we show the statistics results for LASSO method when we used EVI and VOD data for provide the best results and become aware about how the method combined the two indices.  LASSO results are similar to RLR results but using less features. 


\begin{figure}[t!]
\centering
\vspace{-1cm}
	\includegraphics[scale = 0.25]{figures/weight/weight_variables_EVI_VOD_LASSO_Oct.pdf}
	\includegraphics[scale = 0.25]{figures/weight/weight_variables_EVI_VOD_corn_Oct.pdf}\\
		\includegraphics[scale = 0.25]{figures/weight/weight_variables_EVI_VOD_soybeans_Oct.pdf}
			\includegraphics[scale = 0.25]{figures/weight/weight_variables_EVI_VOD_wheat_Oct.pdf}\\

    \caption{Graphs with the importance of each variable for LASSO method. For each experiment we show two graphs with the mean of time series and the weight established for LASSO method for both vegetation index (EVI and VOD). (Top-Left) all crops, (Top-Right) corn experiment, (Down-Left) soybean experiment and (Down-Right) wheat experiment. }
    \label{fig:weigthLASSO}
\end{figure}

 \begin{figure}[h!]
\centering
\vspace{-1cm}
	\includegraphics[scale = 0.25]{figures/RLR/weight_variables_allcrops_Oct.pdf}
	\includegraphics[scale = 0.25]{figures/RLR/weight_variables_EVI_VOD_corn_Oct.pdf}\\
		\includegraphics[scale = 0.25]{figures/RLR/weight_variables_EVI_VOD_soybeans_Oct.pdf}
			\includegraphics[scale = 0.25]{figures/RLR/weight_variables_EVI_VOD_wheat_Oct.pdf}\\

    \caption{Graphs with the importance of each variable for RLR method. For each experiment we show two graphs with the mean of time series and the weight established for RLR method for both vegetation index (EVI and VOD). (Top-Left) all crops, (Top-Right) corn experiment, (Down-Left) soybean experiment and (Down-Right) wheat experiment. }
    \label{fig:weightRLR}
\end{figure}

\begin{table}[t!] \centering %
\caption{Statistical results for all experiments: ME (x1000) [Kg$\cdot$m$^{-2}$], RMSE (x100) [Kg$\cdot$ m$^{-2}$] and R$^2$. }
\begin{tabular}{c c|c|c|c}
\hline \hline
\multicolumn{1}{c}{Model} &\multicolumn{1}{c}{\#crop}  & \multicolumn{3}{|c}{LASSO}  \\
\hline
& & {ME} & {RMSE} & {R$^2$}   \\
\hline\hline
EVI \& VOD & All crops&-1.92 $\pm$ 12.16&9.16 $\pm$ 0.94&0.82 $\pm$ 0.04 \\
EVI \& VOD& Corn & -0.4 $\pm$ 5.3&6.13 $\pm$ 0.46&0.89 $\pm$ 0.01 \\
EVI \& VOD& Soybean &-1.3 $\pm$ 1.88&2.1 $\pm$ 0.15&0.88 $\pm$ 0.02 \\
EVI \& VOD& Wheat &-4.56 $\pm$ 11.28&6.12 $\pm$ 0.72&0.58 $\pm$ 0.07 \\
EVI \& VOD& 194 Wheat&-0.26 $\pm$ 7.77&5.96 $\pm$ 0.58&0.6 $\pm$ 0.09 \\
\hline\hline
\end{tabular}
\label{tab:resultsLASSO}
\end{table}



We used the time-series of vegetation indices without phenological information. In Fig. \ref{fig:weigthLASSO}, we can see the feature importance for the whole EVI and VOD time series data from April to October of 2015. We show the weights of LASSO method in all experiments with green bars and analyzed which dates have the most influence in the predictions. In addition, we analyzed if the method is able to highlight dates related with the phenological stages. For each experiment we show two different graphs with the mean time series of all counties used and the weight of each vegetation index, EVI and VOD. We can see how the weight distribution changes for each different experiment. Thus, the weight associated to each feature depends on the type of crop.

First experiment with total yield focuses the high weights after 15th of July, while the others experiments with a unique crop also attach importance to other regions. For each crop we have different important dates. 
While corn crop give greater weight before September dates, soybean and wheat crops expand the important dates along all time series, more especially wheat crop. Probably, this behaviour is due to the influence of the planting dates of winter wheat by the end of September. 
It should be underlined that the wheat crop is the unique experiment that provided greater weight to VOD dates than EVI dates. Only corn experiment has the same range of weight than total yield experiment, surely due to the reason to be the crop with the largest number of counties and total production.


------------------------------------------------------------------------\\
Crop proportion (maximum alphas in KRR problem):\\
County number 310 with alpha 9.1587 and yield 0.2713\\
Corn \%: 0. Soybean \%: 21.1093. Wheat \%: 40.5629\\
County number 316 with alpha 8.4146 and yield 0.44986\\
Corn \%: 22.5255. Soybean \%: 45.4949. Wheat \%: 20.1953\\
County number 329 with alpha 8.2643 and yield 0.66731\\
Corn \%: 46.4859. Soybean \%: 45.7665. Wheat \%: 7.7476\\
County number 341 with alpha 8.1502 and yield 0.62334\\
Corn \%: 39.5747. Soybean \%: 54.7549. Wheat \%: 5.6704\\
------------------------------------------------------------------------\\
Crop proportion (minimum alphas):\\
County number 131 with alpha 0.00059351 and yield 0.83912\\
Corn\%: 57.988. Soybean \%: 41.7781. Wheat \%: 0\\
County number 38 with alpha 0.000731 and yield 0.91874\\
Corn \%: 54.8091. Soybean \%: 44.9081. Wheat \%: 0.28289\\
County number 343 with alpha 0.0029839 and yield 0.60257\\
Corn \%: 41.9463. Soybean \%: 51.1186. Wheat \%: 6.9351\\
County number 322 with alpha 0.0031946 and yield 0.54151\\
Corn \%: 41.1899. Soybean \%: 51.8307. Wheat \%: 6.9794\\
------------------------------------------------------------------------


 \begin{figure}[h!]
\centering
\vspace{-0.5cm}
	\includegraphics[scale = 0.5]{figures/maps/weight_KRR_allcrops.png}\\
	\vspace{-0.5cm}
    \caption{Map with weight in KRR model in total yield crops}
    \label{fig:weigthKRR}
\end{figure}



\red{PERMUTATION RESULTS}

 \begin{figure}[h!]
\centering
\vspace{-0.5cm}
	\includegraphics[scale = 0.5]{figures/weight/permutationRLR_EVI_VOD_Oct.pdf}\\
	\vspace{-0.5cm}
    \caption{permutation RLR}
    \label{fig:permutationRLR}
\end{figure}
 \begin{figure}[h!]
\centering
\vspace{-0.5cm}
	\includegraphics[scale = 0.5]{figures/weight/permutationKRR_EVI_VOD_Oct.pdf}\\
	\vspace{-0.5cm}
    \caption{permutation KRR}
    \label{fig:permutation KRR}
\end{figure}







